packetLSTM: Dynamic LSTM Framework for Streaming Data with Varying Feature Space

We study the online learning problem characterized by the varying input feature space of streaming data. Although LSTMs have been employed to effectively capture the temporal nature of streaming data, they cannot handle the dimension-varying streams in an online learning setting. Therefore, we propose a dynamic LSTM-based novel method, called packetLSTM, to model the dimension-varying streams. The packetLSTM's dynamic framework consists of an evolving packet of LSTMs, each dedicated to processing one input feature. Each LSTM retains the local information of its corresponding feature, while a shared common memory consolidates global information. This configuration facilitates continuous learning and mitigates the issue of forgetting, even when certain features are absent for extended time periods. The idea of utilizing one LSTM per feature coupled with a dimension-invariant operator for information aggregation enhances the dynamic nature of packetLSTM. This dynamic nature is evidenced by the model's ability to activate, deactivate, and add new LSTMs as required, thus seamlessly accommodating varying input dimensions. The packetLSTM achieves state-of-the-art results on five datasets, and its underlying principle is extended to other RNN types, like GRU and vanilla RNN.

==> FigureTex/Fig_DataDepiction.tex <==
\begin{figure}[th]
    \begin{center}
    \includegraphics[width=.65\textwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm}, clip]{Figure/DataDepiction.pdf} 
    \end{center}
    \caption{A snapshot of haphazard inputs and their associated characteristics.}
    \label{fig:data}
\end{figure}

==> FigureTex/Fig_Dataset_Combination.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=\textwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm}, clip]{Figure/dataset_combination.png} 
    \end{center}
    \caption{packetLSTM on different characteristics of haphazard inputs compared to other methods.}
    \label{fig:data_combination}
\end{figure}

==> FigureTex/Fig_radar.tex <==
\begin{figure}[th]
    \begin{center}
    \includegraphics[width=\textwidth, trim={0.0cm 0.0cm 0.0cm 0.0cm}, clip]{Figure/chart.png} 
    \end{center}
    \caption{Performance comparison of packetLSTM with other models.}
    \label{fig:radar}
\end{figure}

==> Tables/tab_ablation_try.tex <==
\begin{table}
    \caption{Ablation study on the architecture of packetLSTM. We consider two experiments to have similar performance if the difference between their mean balanced accuracy is less or equal to 0.05. Here, w stands for the number of wins.}
    \label{tab:ablation}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{rlcp{.01mm}cccp{.01mm}cp{.01mm}cccp{.01mm}cccp{.01mm}ccc}
    \toprule
     & \multirow{2}{*}{Characteristics} & \multirow{2}{*}{\textit{w}} & {} & \multicolumn{3}{c}{magic04} & {} & \multirow{2}{*}{imdb} & {} & \multicolumn{3}{c}{a8a} & {} & \multicolumn{3}{c}{SUSY} & {} & \multicolumn{3}{c}{HIGGS} \\
    \cmidrule{5-7}
    \cmidrule{11-13}
    \cmidrule{15-17}
    \cmidrule{19-21}
    & & & {} & 25 & 50 & 75 & {} & & {} & 25 & 50 & 75 & {} & 25 & 50 & 75 & {} & 25 & 50 & 75 \\
    \midrule
    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{Agg}}}}}} & Mean & 3 & & 60.98 & 67.06 & 72.30 & {} &
    \textbf{85.06} & {} & 58.52 & 65.15 & 67.50 & {} & \textbf{63.16} & \textbf{69.59}  & 74.07 & {} & 52.01 & 55.27 & 58.04 \\
    & Sum & 5 &  & 61.27 & 67.93 & 73.21 & {} & 83.63 & {} & 58.26 & 65.15 & 68.80 & {} & \textbf{63.19} & 69.29 & \textbf{74.39} & {} & \textbf{52.24} & \textbf{55.64} & \textbf{59.06} \\
    & Min & 6 &  & \textbf{61.36} & \textbf{68.28} & 73.58 & {} & 77.64 & {} & \textbf{60.53} & \textbf{67.78} & \textbf{71.13} & {} & 62.78 & 69.29 & 73.85 & {} & \textbf{52.21} & 55.50 & 58.70 \\
    & Max & 7 &  & \textbf{61.33} & \textbf{68.31} & \textbf{73.64} & {} & 77.90 & {} &  \textbf{60.53} & \textbf{67.73} & \textbf{71.11} & {} & 62.77 & 69.28 & 73.85 & {} & \textbf{52.22} & 55.47 & 58.71 \\
    \midrule
    
    \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{Time Model}}}}}} & None  & 0 & & 58.83 & 65.12 & 69.87 & {} & 85.18  & {} & 58.77  & 66.52  & 70.30  & {} & 62.30  & 68.70  & 73.25  & {} & 51.37  & 54.05  &57.06 \\
    & Decay & 1 & & 58.73  & 64.99 & 69.81 & {} & \textbf{85.30} & {} & 58.82  & 67.14  & 70.76  & {} & 62.37  & 68.89  & 73.40  & {} & 51.41  & 54.09  &57.01 \\
    & TimeLSTM-1 & 8 & & 61.13  & 68.14 & \textbf{73.63} & {} & 85.06  & {} & 60.45  & 67.63  & \textbf{71.09} & {} & \textbf{62.77} & \textbf{69.33} & \textbf{73.91} & {} & \textbf{52.23} & \textbf{55.53} & \textbf{58.70} \\
    & TimeLSTM-2 & 9 & & \textbf{61.32} & \textbf{68.34} & \textbf{73.65} & {} & 85.15 & {} & 60.33 & 67.62 & \textbf{71.09} & {} & \textbf{62.79} & \textbf{69.31} & \textbf{73.88} & {} & \textbf{52.26} & \textbf{55.53} & 58.65 \\
    & TimeLSTM-3 & 10 & & \textbf{61.33} & \textbf{68.31} & \textbf{73.64} & {} & 85.06 & {} &  \textbf{60.53} & \textbf{67.73} & \textbf{71.11} & {} & \textbf{62.77} & \textbf{69.28} & 73.85 & {} & \textbf{52.22} & 55.47 & \textbf{58.71} \\
    \midrule

    \parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{Feat}}}}}} & Universal  & 11 & & \textbf{61.37} & \textbf{68.33} & \textbf{73.69} & {} & \textbf{85.06} & {} & 60.32 & 67.58 & \textbf{71.15} & {} & \textbf{62.79} & \textbf{69.27} & \textbf{73.84} & {} & \textbf{52.26} & \textbf{55.52} & \textbf{58.69} \\
    & Current & 13 & & \textbf{61.33} & \textbf{68.31} & \textbf{73.64} & {} & \textbf{85.06} & {} &  \textbf{60.53} & \textbf{67.73} & \textbf{71.11} & {} &  \textbf{62.77} & \textbf{69.28} & \textbf{73.85} & {} & \textbf{52.22} & \textbf{55.47} & \textbf{58.71} \\
    \midrule

    \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{Concat}}}}}} & Only LTM  & 5 & & 60.94 & 67.66 & 73.09& {} & \textbf{85.15} & {} & 59.36 & 66.86 & 70.34 & {} & \textbf{62.78} & \textbf{69.32} &  \textbf{73.85} & {} & \textbf{52.20} & 52.62 & 57.69 \\
    & Only STM & 5 & & 61.15 & \textbf{68.26} & 73.38& {} & \textbf{85.17} & {} & 60.02 & 67.57 & 70.77 & {} & \textbf{62.82} & \textbf{69.33} & \textbf{73.89} & {} & \textbf{52.18} & 52.19 & 57.63\\
    & Both & 12 & & \textbf{61.33} & \textbf{68.31} & \textbf{73.64} & {} & 85.06 & {} &  \textbf{60.53} & \textbf{67.73} & \textbf{71.11} & {} & \textbf{62.77} & \textbf{69.28} & \textbf{73.85} & {} & \textbf{52.22} & \textbf{55.47} & \textbf{58.71} \\
    \midrule

    
    \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{Normalization}}}}}} & None  & 4 & & 59.14 & 65.44& 70.53& {} & \textbf{85.61} & {} & 59.97 & \textbf{67.89} & \textbf{71.22} & {} & 63.12 & \textbf{69.65} & 74.19 & {} & 51.46 & 54.33 & 57.39 \\
    & Min Max & 0 & & 57.69 & 63.33 & 68.42 & {} & 85.23  & {} & 59.94  & 67.76  & 71.15  & {} & 62.37  & 69.06  & 73.61  & {} & 51.21  & 53.10  & 55.52 \\
    & Decimal Scaling & 0 & & 55.03  & 60.36 & 65.72 & {} & 85.23  & {} & 49.99  & 50.00  & 50.00  & {} & 50.96  & 58.53  & 63.31  & {} & 50.00  & 50.00  & 50.00 \\
    & Mean Norm & 3 & & 60.23  & 66.71 & 71.86 & {} & 84.89  & {} & 58.03  & 65.94  & 70.07  & {} & \textbf{63.19} & \textbf{69.68} & \textbf{74.31} & {} & 51.86  & 54.88  & 58.11 \\
    & Unit Vector & 0 & & 50.01  & 54.23 & 60.02 & {} & 85.32  & {} & 58.12  & 65.67  & 68.97  & {} & 56.52  & 65.43  & 71.44  & {} & 50.75  & 52.86  &55.53 \\
    & Z-score & 7 & & \textbf{61.33} & \textbf{68.31} & \textbf{73.64} & {} & 85.06 & {} & \textbf{60.53} & 67.73  & 71.11  & {} & 62.77  & 69.28  & 73.85 & {} & \textbf{52.22} & \textbf{55.47} & \textbf{58.71} \\
    \midrule

    \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\underline{\texttt{\small{RNN}}}}}} & Vanilla RNN  & 9 & & \textbf{60.50} & \textbf{66.77} & \textbf{71.85} & {} & 82.83 & {} & 50.00 & 60.48 & 68.03 & {}   & \textbf{62.84} & \textbf{69.34} & \textbf{73.98} & {} & \textbf{51.95} & \textbf{54.71} & \textbf{57.62} \\
    & GRU & 1 & & 60.34 & 66.24 & 71.23 & {} & 81.49 & {} & 50.96  & 60.86  & \textbf{73.38} & {} & 62.73  & 69.16  & 73.72 & {} & 51.80  & 54.25  & 56.79  \\
    & LSTM & 3 & & 58.83  & 65.12 & 69.87 & {} & \textbf{85.18} & {} & \textbf{58.77} & \textbf{66.52} & 70.30  & {} & 62.30  & 68.70  & 73.25  & {} & 51.37  & 54.05  & 57.06 \\

    
    \bottomrule
    \end{tabular}
    }
\end{table}

==> Tables/tab_dataset_description.tex <==
\begin{table}[]
    \caption{Dataset Description: \# \{Instances, Features\} represents the number of \{Instances, Features\}.}
    \label{tab:dataset_description}
    \centering
    \begin{tabular}{r|ccccc}
    \toprule
    Dataset & \# Instances & \# Features & Imbalance & Missing Values \% & Type\\
    \midrule
    magic04 \cite{bock2004methods} & 19020 & 10 & 64.84\% & 25\%, 50\%, 75\% & Synthetic \\
    imdb \cite{maas2011learning} & 25000 & 7500 & 50\% & 98.35\% & Real \\
    a8a \cite{kohavi1996scaling} & 32561 & 123 & 75.92\% & 25\%, 50\%, 75\% & Synthetic \\
    SUSY \cite{baldi2014searching} & 1M & 8 & 45.79\% & 25\%, 50\%, 75\% & Synthetic \\
    HIGGS \cite{baldi2014searching} & 1M & 21 & 52.97\% & 25\%, 50\%, 75\% & Synthetic \\
    \bottomrule
    \end{tabular}
\end{table}

==> Tables/tab_model_characteristics.tex <==
\begin{table}
    \caption{Model performance on different combinations of characteristics}
    \label{tab:model_characteristic}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llclp{.01mm}cccp{.01mm}cp{.01mm}cccp{.01mm}cccp{.01mm}ccc}
    \toprule
    \multirow{2}{*}{Agg} & \multirow{2}{*}{Uni. Feat} & \multirow{2}{*}{Decay} & \multirow{2}{*}{Norm} & {} & \multicolumn{3}{c}{magic04} & {} & \multirow{2}{*}{imdb} & {} & \multicolumn{3}{c}{a8a} & {} & \multicolumn{3}{c}{SUSY} & {} & \multicolumn{3}{c}{HIGGS} \\
    \cmidrule{6-8}
    \cmidrule{12-14}
    \cmidrule{16-18}
    \cmidrule{20-22}
    & & & & {} & 25 & 50 & 75 & {} & & {} & 25 & 50 & 75 & {} & 25 & 50 & 75 & {} & 25 & 50 & 75 \\
    \midrule
    \multirow{4}{*}{Mean} & T & GRU-D & F & {} & 59.22 & 65.38 & 70.42 & {} & 85.53 & {} & 56.75 & 63.86 & 62.06 & {} & 62.97 & 69.35 & 73.71 & {} & 51.27 & 53.89 & 56.57 \\
    & T & F & F & {} & 59.21 & 65.28 & 70.32 & {} & 85.27 & {} & 56.41 & 62.23 & 63.67 & {} & 62.95 & 69.31 & 73.69 & {} & 51.25 & 53.73 & 56.46 \\
    & \textbf{F} & GRU-D & F & {} & 59.21 & 65.41 & 70.36 & {} & 85.50 & {} & 57.34 & 64.40 & 61.01 & {} & 62.90 & 69.36 & 73.72 & {} & 51.21 & 53.89 & 56.55 \\
    & F & F & F & {} & 59.26 & 65.32 & 70.28 & {} & 85.40 & {} & 56.48 & 62.56 & 63.84 & {} & 62.88 & 69.32 & 73.69 & {} & 51.18 & 53.72 & 56.42 \\
    \midrule
    \multirow{4}{*}{Max} & T & GRU-D & F & {} & 58.65 & 65.00 & 69.87 & {} & 73.04 & {} & 58.85 & 66.96 & 70.61 & {} & 63.07 & 69.58 & 74.11 & & 51.42 &  54.09& 57.16 \\
    & T & F & F & {} & 58.60 & 65.01 & 69.92 & {} & 72.94 & {} & 58.68 & 66.67 & 70.16 & {} & 63.04 & 69.53 & 74.06 & & 51.35&  53.97 & 57.04 \\
    & \textbf{F} & GRU-D & F & {} & 58.73 & 64.99 & 69.84 & {} & 73.06 & {} & 58.77 & 66.92 & 70.61 & {} & 63.06 & 69.56 & 74.12 & & 51.39 & 54.07 & 57.12 \\
    & F & F & F & {} & 58.74 & 64.85 & 69.78 & {} & 72.95 & {} & 58.62 & 66.72 & 70.16 & {} & 63.04 & 69.53 & 74.06 & & 51.38 & 54.00 & 56.99 \\
    \midrule
    & F & \textbf{T-3} & F & {} & 59.42 & 65.58 & 70.46 & {} & 85.65 & {} & 59.97 & 67.89 & 71.22 & {} & 63.12 & 69.65& 74.19 & {} & 51.46 & 54.33 & 57.39\\
    & F & T-2 & F & {} & 59.25 & 65.65 & 70.56 & {} & 85.58 & {} & 59.77 & 67.70 & 71.26 & {} &63.13 & 69.64& 74.20 & {} & 51.47 & 54.37 & 57.45\\
    & F & T-1 & F & {} & 59.21 & 65.41 & 70.36 & {} & 84.50 & {} & 58.77 & 66.92 & 70.61 & {} & 63.13 & 69.65 & 74.21 & {} & 51.46\\
    \midrule
    Mean (range L1) & F & T-3 & F & {} & 59.42 & 65.58 & 70.46 & {} & 85.65 & {} & 57.86 & 64.92 & 67.59 & {} &62.97 & 69.39 & 73.78 & {} & 51.26& 53.97 & 56.56\\
    Max & F & T-3 & F & {} & 59.16 & 65.65 & 70.59 & {} & 77.07 & {} & 59.97 & 67.89 & 71.22 & {} & 63.12 & 69.65 & 74.19 & {} & 51.46 & 54.33 & 57.39\\
    Min & F & T-3  & F & {} & 59.12 & 65.59 & 70.34 & {} & 76.67 & {} & 59.73 & 67.83 & 71.12 & {} & 63.12& 69.65 & 74.20 & {} & 51.46 & 54.47& 57.44\\
    Sum (L1) & F & T-3  & F & {} & 59.60 & 65.86 & 70.85 & {} & 84.76 & {} & 58.04 & 66.17 & 62.05 & {} & 63.07 & 69.59& 74.12& {} & 51.53 & 54.67 & 57.86 \\
    L2 & F & T-3  & F & {} & & & & {} & & {} & 59.59 & 67.37 & 71.00 & {} & & &74.01 & {} & & & 57.19\\
    Range L2 & F & T-3  & F & {} & & & & {} & & {} & 53.61 & 62.15 & 64.72 & {} & & & 73.85 & {} & & & 55.67\\
    \multicolumn{4}{c}{\textbf{Best Aggregator}} & {} & Sum & Sum & Sum & {} & Mean & {} & Max & Max & Max & {} & Max & Max & Max & {} & Sum & Sum & Sum \\
    \midrule
    \multicolumn{21}{c}{\textbf{Finding Best Normalization}}\\
     \midrule
     Mean & F & T-3 & Off. & {} & 60.87 & 67.06 & 72.15 & {} &  & {} &  61.46 & 68.39 & 71.35 & {} & \\
     Max & F & T-3 & Off. & {} & 61.34 & 68.34 & 73.69 & {} &  &{} & 61.94 & 69.51 & 72.46 & {} & 63.24 & 69.80 & 74.39 & {} & 52.24 & 55.52 & 58.81  \\
     Sum & F & T-3 & Off. & {} & 61.25 & 67.95 & 73.13 & {} &  &{} & 61.19 & 68.14 & 71.33 & {} & 63.17 & 69.79 & 74.39  & {} & 52.25 & 55.63 & 59.04 \\
    \midrule
     \multirow{7}{*}{Sum} & F & T-3 & Min-Max  & {} & 58.06 & 64.30 & 69.47 & {} &  &{} & & & & {} &62.22 &68.69 &74.21 & {} & & & \\
     & F & T-3 & Z-score  & {} & 61.23 & 67.92 & 73.14 & {} &  & {} & & 66.26 & 67.13 & {} & 63.19 &69.79 &74.39 & {} & 52.24 &55.63 &59.05 \\
     & F & T-3 & Dec Scal & {} & 56.04 & 61.81 & 66.42 & {} &  &{} & & & & {} &57.16 &63.59 &68.64 & {} & 50.0 & 50.0&50.0   \\
     & F & T-3 & Mean-Norm & {} & 60.39 & 66.84 & 71.91 & {} &  &{} & & & & {} & 63.11&69.68 &<ran> & {} & (51.81) & (54.91) & (58.33)  \\
     & F & T-3 & Unit-vec & {} & 50.00 & 54.63 & 61.49 & {} &  &{} & & & & {} & 56.80&66.05 &72.15 & {} & 50.67  & 53.35 & 56.23  \\
     & F & T-3 & t-Digest & \\
     \midrule
     \multirow{7}{*}{Max} & F & T-3 & Min-Max  & {} & 57.65 & & & {} &  &{} & & & & {} & 62.37&  69.06& 73.61 & {}& <ran>& & \\
     & F & T-3 & Z-score  & {} & 61.32 & 68.36 & 73.65 & {} &  & {} & 60.33 & 67.73 & 71.23 & {} & 63.25& 69.81 &74.40  & {} & 52.27 &55.49 &58.67 \\
     & F & T-3 & Dec Scal &{} & & & & {} &  &{} & & & & {} &  &  &  & {} &  \\
     & F & T-3 & Mean-Norm &{} & & & & {} &  &{} & & & & {} &63.19 & 69.77& 74.31 & {} & \\
     & F & T-3 & Unit-vec &{} & & & & {} &  &{} & & & & {} &  & &  & {} &  \\
     & F & T-3 & t-Digest & \\
     \midrule
     \multirow{7}{*}{Mean} & F & T-3 & Min-Max  &{} & & & & {} &  &{} & & & & {} & \\
     & F & T-3 & Z-score  &{} & & & & {} & 85.11 &{} & & & & {} &  \\
     & F & T-3 & Dec Scal &{} & & & & {} &  &{} & & & & {} &  \\
     & F & T-3 & Mean-Norm &{} & & & & {} &  &{} & & & & {} &  \\
     & F & T-3 & Unit-vec &{} & & & & {} &  &{} & & & & {} &    \\
     & F & T-3 & t-Digest & \\
     \midrule
     \multicolumn{21}{c}{\textbf{Class Imbalance}}\\
     \midrule
     Max (\textbf{Offline}) & F & T-3 & Z-score & {} & 61.32 & 68.35 & 73.70 & {} & & {} & 60.33 & 67.73 & 71.23 & {} & \\
     Max (\textbf{Online}) & F & T-3 & Z-score & {} & 61.32 & 68.36 & 73.69 & {} & & {} & 60.32 & 67.78 & 71.26 & {} & 63.25 & 69.82& 74.40 & {} & 52.24 & 55.51& 58.73\\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> Tables/tab_results.tex <==
\begin{table*}[!th]
  \caption{Comparison of models on all datasets. The deterministic models --- NB3, FAE, and OLVF --- underwent a single execution and the non-deterministic models were executed 5 times, with the mean $\pm$ standard deviation reported. A \textsuperscript{$\ddagger$} symbol indicates non-deterministic models that were run only once on specific datasets due to substantial time constraints. The bAcc stands for balanced Accuracy, and \textsuperscript{$\dagger$} denotes the real datasets.}
  \label{tab:results}
  \centering
  \resizebox{\linewidth}{!}{%
  % \begin{adjustbox}{width=\linewidth,center}
  \begin{tabular}{lccccccccccc}
  % \vspace{2em}
  \toprule
  Dataset & $p$ & NB3 & FAE & OLVF & OCDS & OVFM & DynFo & ORF\textsuperscript{3}V & Aux-Net & Aux-Drop & \textbf{Our}\\
  \midrule

  \multirow{3}{*}{magic04} & 
  0.25 & 50.01 & 50.01 & 53.18 & 51.89$\pm$0.10 & 51.94$\pm$0.00 & 52.75$\pm$0.30	& 47.94$\pm$0.22 & 50.09$\pm$0.07 & 56.04$\pm$0.53 & \textbf{61.33$\pm$0.07} \\
  &  0.50 & 50.02 & 50.00 & 54.6 & 53.40$\pm$0.45	& 54.13$\pm$0.08 &	55.12$\pm$0.06	& 48.56$\pm$0.11 & 50.09$\pm$0.03 & 59.29$\pm$0.48 & \textbf{68.31$\pm$0.15}	 \\ 
  &  0.75 & 49.99 & 50.00	& 56.19	& 53.76$\pm$1.07 & 58.79$\pm$0.04	& 56.75$\pm$0.02 & 49.32$\pm$0.04 & 50.05$\pm$0.07 & 63.18$\pm$0.61	& \textbf{73.64$\pm$0.11} \\
  \midrule
  
 imdb\textsuperscript{$\dagger$} &
    & 81.56 & 82.18 & 80.08 & 50.14$\pm$0.02 & \textsuperscript{$\ddagger$} & 57.98$\pm$0.29 & 76.47$\pm$0.11 & 67.41\textsuperscript{$\ddagger$} & 73.10$\pm$0.19 & \textbf{85.06$\pm$0.04} \\
  \midrule
  
  \multirow{3}{*}{a8a} & 
   0.25& 50.01 & 50.00	& \textbf{60.67} & 54.75$\pm$0.87 & 58.66$\pm$0.00 & 50.01$\pm$0.03	& 49.99$\pm$0.00 & 50.00$\pm$0.00 & 50.00$\pm$0.01 &  60.53$\pm$0.16\\
  &  0.50 & 50.01 & 50.00 & 66.46 & 64.04$\pm$1.01 & 66.02$\pm$0.00 & 50.11$\pm$0.01 & 50.01$\pm$0.00 & 50.00$\pm$0.00 & 55.33$\pm$1.99 & \textbf{67.73$\pm$0.21} \\
  &  0.75& 50.01 & 50.00	& 70.6 & 68.81$\pm$1.10 & 70.95$\pm$0.00	& 50.13$\pm$0.01 & 49.99$\pm$0.00	& 50.00$\pm$0.00 & 62.87$\pm$0.93 & \textbf{71.11$\pm$0.16} \\
  \midrule


  \multirow{3}{*}{SUSY} & 
   0.25 & 50.00 &   49.90    & 51.12	 & 52.11$\pm$0.19 & 58.00$\pm$0.00 & 54.69$\pm$0.01 & 49.37$\pm$0.01	& 50.53$\pm$1.17 & 61.98$\pm$0.10 & \textbf{62.77$\pm$0.01} \\
  &  0.50 & 50.00	& 50.01 & 53.21	& 54.03$\pm$0.28 & 62.85$\pm$0.00 & 58.27$\pm$0.00 & 48.33$\pm$0.02 & 57.89$\pm$7.19 & 68.79$\pm$0.14 & \textbf{69.28$\pm$0.01} \\
  &  0.75 & 50.00 & 50.12	& 55.98	& 54.84$\pm$0.48 & 68.51$\pm$0.00	& 60.94$\pm$0.01 & 47.53$\pm$0.03 & 53.67$\pm$8.13 & 73.55$\pm$0.11 & \textbf{73.85$\pm$0.02} \\
  \midrule

  \multirow{3}{*}{HIGGS} & 
   0.25 & 50.00 &   50.16 & 50.57 & 49.97$\pm$0.07	& 50.61$\pm$0.01 & 50.18\textsuperscript{$\ddagger$} & 49.86$\pm$0.03 & 49.99$\pm$0.00 & 51.17$\pm$0.05 & \textbf{52.22$\pm$0.04} \\
  &  0.50 & 50.00 & 50.01 & 51.21	& 50.06$\pm$0.06 & 51.40$\pm$0.01 & 50.21\textsuperscript{$\ddagger$} & 49.82$\pm$0.02 & 49.99$\pm$0.01	& 53.09$\pm$0.05 & \textbf{55.47$\pm$0.04} \\
  &  0.75& 50.00	& 50.55	& 51.98	& 49.97$\pm$0.05 & 52.66$\pm$0.00	& 50.16\textsuperscript{$\ddagger$} & 49.75$\pm$0.03 & 49.98\textsuperscript{$\ddagger$} & 55.55$\pm$0.11&	\textbf{58.71$\pm$0.05} \\

  \bottomrule
  \end{tabular}  
  }
  % \end{adjustbox}
\end{table*}

==> Tables/tab_results_with_per_improve_0.tex <==
\begin{table*}[!t]
  \caption{Comparison of models on all datasets based on balanced accuracy. The deterministic models --- NB3, FAE, OLVF, and OLIFL --- underwent a single execution, and the non-deterministic models were executed 5 times, with the mean $\pm$ standard deviation reported. A \textsuperscript{$\ddagger$} symbol indicates non-deterministic models that were run only once on specific datasets due to substantial time constraints, and \textsuperscript{$\dagger$} denotes the real datasets. \% Im. denotes the \% improvement in the performance of packetLSTM compared to the previous best-performing baseline (denoted by italics) in each dataset.}
  \vspace{0.5em}
  \label{tab:results}
  \centering
  \resizebox{\linewidth}{!}{%
  % \begin{adjustbox}{width=\linewidth,center}
  \begin{tabular}{lcccccccccccc|r}
  \toprule
  Dataset & $p$ & NB3 & FAE & OLVF & OLIFL & OCDS & OVFM & DynFo & ORF\textsuperscript{3}V & Aux-Net & Aux-Drop & \textbf{packetLSTM} & \textit{\% Im.} \\
  \midrule

  \multirow{3}{*}{magic04} & 
  0.25 & 50.01 & 50.01 & 53.18 & 53.06 & 51.89$\pm$0.10 & 51.94$\pm$0.00 & 52.75$\pm$0.30	& 47.94$\pm$0.22 & 50.09$\pm$0.07 & 56.04$\pm$0.53 & \textbf{61.33$\pm$0.07} & \textit{9.44} \\
  &  0.50 & 50.02 & 50.00 & 54.60 & 57.28 & 53.40$\pm$0.45	& 54.13$\pm$0.08 &	55.12$\pm$0.06	& 48.56$\pm$0.11 & 50.09$\pm$0.03 & 59.29$\pm$0.48 & \textbf{68.31$\pm$0.15}	 & \textit{15.21} \\ 
  &  0.75 & 49.99 & 50.00	& 56.19	& 60.75 & 53.76$\pm$1.07 & 58.79$\pm$0.04	& 56.75$\pm$0.02 & 49.32$\pm$0.04 & 50.05$\pm$0.07 & 63.18$\pm$0.61	& \textbf{73.64$\pm$0.11} & \textit{16.56} \\
  \midrule
  
 imdb\textsuperscript{$\dagger$} &
    & 81.56 & 82.18 & 80.08 & 54.36 & 50.14$\pm$0.02 & 77.43\textsuperscript{$\ddagger$} & 57.98$\pm$0.29 & 76.47$\pm$0.11 & 67.41\textsuperscript{$\ddagger$} & 73.10$\pm$0.19 & \textbf{85.06$\pm$0.04} & \textit{3.50} \\
  \midrule
  
  \multirow{3}{*}{a8a} & 
   0.25& 50.01 & 50.00	& \textbf{60.67} & 53.57 & 54.75$\pm$0.87 & 58.66$\pm$0.00 & 50.01$\pm$0.03	& 49.99$\pm$0.00 & 50.00$\pm$0.00 & 50.00$\pm$0.01 &  60.53$\pm$0.16 & \textit{-0.23} \\
  &  0.50 & 50.01 & 50.00 &  66.46  & 54.63 & 64.04$\pm$1.01 & 66.02$\pm$0.00 & 50.11$\pm$0.01 & 50.01$\pm$0.00 & 50.00$\pm$0.00 & 55.33$\pm$1.99 & \textbf{67.73$\pm$0.21} & \textit{1.91} \\
  &  0.75& 50.01 & 50.00	 & 70.60  & 56.56 & 68.81$\pm$1.10 & 70.95$\pm$0.00	& 50.13$\pm$0.01 & 49.99$\pm$0.00	& 50.00$\pm$0.00 & 62.87$\pm$0.93 & \textbf{71.11$\pm$0.16} & \textit{0.23} \\
  \midrule


  \multirow{3}{*}{SUSY} & 
   0.25 & 50.00 &   49.90    & 51.12  & 51.23	 & 52.11$\pm$0.19 & 58.00$\pm$0.00 & 54.69$\pm$0.01 & 49.37$\pm$0.01	& 50.53$\pm$1.17 & 61.98$\pm$0.10 & \textbf{62.77$\pm$0.01} & \textit{1.27} \\
  &  0.50 & 50.00	& 50.01 & 53.21	& 53.59 & 54.03$\pm$0.28 & 62.85$\pm$0.00 & 58.27$\pm$0.00 & 48.33$\pm$0.02 & 57.89$\pm$7.19 & 68.79$\pm$0.14 & \textbf{69.28$\pm$0.01} & \textit{0.71} \\
  &  0.75 & 50.00 & 50.12	& 55.98	& 56.39 & 54.84$\pm$0.48 & 68.51$\pm$0.00	& 60.94$\pm$0.01 & 47.53$\pm$0.03 & 53.67$\pm$8.13 & 73.55$\pm$0.11 & \textbf{73.85$\pm$0.02} & \textit{0.41} \\
  \midrule

  \multirow{3}{*}{HIGGS} & 
   0.25 & 50.00 &   50.16 & 50.57 & 50.56 & 49.97$\pm$0.07	& 50.61$\pm$0.01 & 50.18\textsuperscript{$\ddagger$} & 49.86$\pm$0.03 & 49.99$\pm$0.00 & 51.17$\pm$0.05 & \textbf{52.22$\pm$0.04} & \textit{2.05} \\
  &  0.50 & 50.00 & 50.01 & 51.21	& 51.50 & 50.06$\pm$0.06 & 51.40$\pm$0.01 & 50.21\textsuperscript{$\ddagger$} & 49.82$\pm$0.02 & 49.99$\pm$0.01	& 53.09$\pm$0.05 & \textbf{55.47$\pm$0.04} & \textit{4.48} \\
  &  0.75& 50.00	& 50.55	& 51.98	& 52.48 & 49.97$\pm$0.05 & 52.66$\pm$0.00	& 50.16\textsuperscript{$\ddagger$} & 49.75$\pm$0.03 & 49.98\textsuperscript{$\ddagger$} & 55.55$\pm$0.11&	\textbf{58.71$\pm$0.05} & \textit{5.69} \\

  \bottomrule
  \end{tabular}  
  }
  % \end{adjustbox}
\end{table*}
